Spectral Clustering for Optical Confirmation and Redshift Estimation of X-ray Selected Galaxy Cluster Candidates in the SDSS Stripe 82

We develop a galaxy cluster finding algorithm based on spectral clustering technique to identify optical counterparts and estimate optical redshifts for X-ray selected cluster candidates. As an application, we run our algorithm on a sample of X-ray cluster candidates selected from the third XMM-Newton serendipitous source catalog (3XMM-DR5) that are located in the Stripe 82 of the Sloan Digital Sky Survey (SDSS). Our method works on galaxies described in the color-magnitude feature space. We begin by examining 45 galaxy clusters with published spectroscopic redshifts in the range of 0.1 to 0.8 with a median of 0.36. As a result, we are able to identify their optical counterparts and estimate their photometric redshifts, which have a typical accuracy of 0.025 and agree with the published ones. Then, we investigate another 40 X-ray cluster candidates (from the same cluster survey) with no redshift information in the literature and found that 12 candidates are considered as galaxy clusters in the redshift range from 0.29 to 0.76 with a median of 0.57. These systems are newly discovered clusters in X-rays and optical data. Among them 7 clusters have spectroscopic redshifts for at least one member galaxy.

==> subfloat.sty.tex <==
%%
%% This is file `subfloat.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% subfloat.dtx  (with options: `package')
%% 
%%   subfloat package
%% 
%%   Copyright  1999 Harald Harders
%% 
%%   This program can be redistributed and/or modified under the terms
%%   of the LaTeX Project Public License Distributed from CTAN
%%   archives in directory macros/latex/base/lppl.txt; either
%%   version 1 of the License, or any later version.
%% 
%%   h.harders@tu-bs.de
%% 
\def\packagename{subfloat}
\def\fileversion{1.03}
\def\filedate{1999/10/08}
\def\docdate{1999/10/08}
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{subfloat}
         [\filedate\space version \fileversion]
\message{Package `subfloat', Version \fileversion\space of \filedate.}
\let\@xp=\expandafter
\let\@nx=\noexpand
\newcounter{parentfigure}% Counter for ``parent figure''.
\newcounter{parenttable}% Counter for ``parent table''.
\newenvironment{subfigures}{%
  \refstepcounter{figure}%
  \begingroup % conservative approach
  \let\protect\@nx
  \edef\@tempa{\def\@nx\theparentfigure{\thefigure}}%
  \@xp\endgroup\@tempa
  \setcounter{parentfigure}{\value{figure}}%
  \setcounter{figure}{0}%
  \def\thefigure{\theparentfigure\alph{figure}}%
  \ignorespaces
}{%
  \setcounter{figure}{\value{parentfigure}}%
  \global\@ignoretrue
}
%%
\newenvironment{subtables}{%
  \refstepcounter{table}%
  \begingroup % conservative approach
  \let\protect\@nx
  \edef\@tempa{\def\@nx\theparenttable{\thetable}}%
  \@xp\endgroup\@tempa
  \setcounter{parenttable}{\value{table}}%
  \setcounter{table}{0}%
  \def\thetable{\theparenttable\alph{table}}%
  \ignorespaces
}{%
  \setcounter{table}{\value{parenttable}}%
  \global\@ignoretrue
}
%%
\newcommand{\subfiguresbegin}{%
  \refstepcounter{figure}%
  \begingroup % conservative approach
  \let\protect\@nx
  \edef\@tempa{\def\@nx\theparentfigure{\thefigure}}%
  \@xp\endgroup\@tempa
  \setcounter{parentfigure}{\value{figure}}%
  \setcounter{figure}{0}%
  \let\theoriginalfigure\thefigure
  \def\thefigure{\theparentfigure\alph{figure}}%
  \ignorespaces
}
%%
\newcommand{\subfiguresend}{%
  \let\thefigure\theoriginalfigure
  \setcounter{figure}{\value{parentfigure}}%
  \global\@ignoretrue
}
%%
\newcommand{\subtablesbegin}{%
  \refstepcounter{table}%
  \begingroup % conservative approach
  \let\protect\@nx
  \edef\@tempa{\def\@nx\theparenttable{\thetable}}%
  \@xp\endgroup\@tempa
  \setcounter{parenttable}{\value{table}}%
  \setcounter{table}{0}%
  \let\theoriginaltable\thetable
  \def\thetable{\theparenttable\alph{table}}%
  \ignorespaces
}
%%
\newcommand{\subtablesend}{%
  \let\thetable\theoriginaltable
  \setcounter{table}{\value{parenttable}}%
  \global\@ignoretrue
}
%%
\endinput
%%
%% End of file `subfloat.sty'.
